A Generic Privacy-Preserving Protocol For Keystroke Dynamics-Based Continuous Authentication

Continuous authentication utilizes automatic recognition of certain user features for seamless and passive authentication without requiring user attention. Such features can be divided into categories of physiological biometrics and behavioral biometrics. Keystroke dynamics is proposed for behavioral biometrics-oriented authentication by recognizing users by means of their typing patterns. However, it has been pointed out that continuous authentication using physiological biometrics and behavior biometrics incur privacy risks, revealing personal characteristics and activities. In this paper, we consider a previously proposed keystroke dynamics-based authentication scheme that has no privacy-preserving properties. In this regard, we propose a generic privacy-preserving version of this authentication scheme in which all user features are encrypted -- preventing disclosure of those to the authentication server. Our scheme is generic in the sense that it assumes homomorphic cryptographic primitives. Authentication is conducted on the basis of encrypted data due to the homomorphic cryptographic properties of our protocol.

==> 3_CA_without_priv.tex <==
%\subsection{Problems with privacy-preserving approaches}\label{sec:ppissue}
%\subsection{Privacy issues}
%As, keystroke dynamics is being utilized for users authentication and verification. Moreover, keystroke dynamics can be used to identify user age, gender and hand used for typing. Due to these reasons, templates of keystroke dynamics need to protected. In this task we propose a method that protects privacy of keystroke dynamics. %(write)


%We assume that the readers have knowledge of cryptographic primitives such as homomorphic encryption and Paillier cryptosystem.


